Browser Feature Usage on the Modern Web

Modern web browsers are incredibly complex, with millions of lines of code and over one thousand JavaScript functions and properties available to website authors. This work investigates how these browser features are used on the modern, open web. We find that JavaScript features differ wildly in popularity, with over 50% of provided features never used in the Alexa 10k. We also look at how popular ad and tracking blockers change the distribution of features used by sites, and identify a set of approximately 10% of features that are disproportionately blocked (prevented from executing by these extensions at least 90% of the time they are used). We additionally find that in the presence of these blockers, over 83% of available features are executed on less than 1% of the most popular 10,000 websites. We additionally measure a variety of aspects of browser feature usage on the web, including how complex sites have become in terms of feature usage, how the length of time a browser feature has been in the browser relates to its usage on the web, and how many security vulnerabilities have been associated with related browser features.

==> figures/megatable.tex <==
\begin{table*}[hp]
  \centering
  \rowcolors{2}{gray!25}{white}
  \begin{tabular}{ l l r r r r }
    \toprule
      Standard Name &
      Abbreviation &
      \multicolumn{1}{c}{\# Features} &
      \multicolumn{1}{c}{\# Sites} &
      \multicolumn{1}{c}{Block Rate} &
      \multicolumn{1}{c}{\# CVEs} \\
    \midrule
      HTML: Canvas                                                  & H-C    & 54    & 7,061   & 33.1\%   & 15 \\
      Scalable Vector Graphics 1.1 (2\textsuperscript{nd} Edition)  & SVG    & 138	  & 1,554   & 86.8\%	 & 14 \\
      WebGL	                                                        & WEBGL  & 136   & 913	    & 60.7\%	 & 13 \\
      HTML: Web Workers	                                            & H-WW   & 2	    & 952	    & 59.9\%	 & 11 \\
      HTML 5		                                                    & HTML5  & 69	  & 7,077	  & 26.2\%	 & 10 \\
      Web Audio API		                                              & WEBA   & 52    & 157	    & 81.1\%   & 10 \\
      WebRTC 1.0                                                    & WRTC   & 28    & 30	    & 29.2\%   & 8 \\
      XMLHttpRequest                                                & AJAX   & 13    & 7,957   & 13.9\%   & 8 \\
      DOM                                                           & DOM    & 36    & 9,088   & 2.0\%    & 4 \\
      Indexed Database API                                          & IDB    & 48    & 302     & 56.3\%   & 3 \\
      Beacon                                                        & BE     & 1     & 2,373   & 83.6\%   & 2 \\
      Media Capture and Streams                                     & MCS    & 4     & 54      & 49.0\%   & 2 \\
      Web Cryptography API                                          & WCR    & 14    & 7,113   & 67.8\%   & 2 \\
      CSSOM View Module                                             & CSS-VM & 28    & 4,833   & 19.0\%   & 1 \\
      Fetch                                                         & F      & 21    & 77      & 33.3\%   & 1 \\
      Gamepad                                                       & GP     & 1     & 3       & 0.0\%    & 1 \\
      High Resolution Time, Level 2                                 & HRT    & 1     & 5,769   & 50.2\%   & 1 \\
      HTML: Web Sockets                                             & H-WS   & 2     & 544     & 64.6\%   & 1 \\
      HTML: Plugins                                                 & H-P    & 10    & 129     & 29.3\%   & 1 \\
      Web Notifications                                             & WN     & 5     & 16      & 0.0\%    & 1 \\
      Resource Timing                                               & RT     & 3     & 786     & 57.5\%   & 1 \\
      Vibration API                                                 & V      & 1     & 1       & 0.0\%    & 1 \\
      Battery Status API                                            & BA     & 2     & 2,579   & 37.3\%   & 0 \\
      % Console API                                                 & CO      & 23    & 4       & 100\%    & 0 \\
      CSS Conditional Rules Module, Level 3                         & CSS-CR & 1     & 449     & 36.5\%   & 0 \\
      CSS Font Loading Module, Level 3                              & CSS-FO & 12    & 2,560   & 33.5\%   & 0 \\
      CSS Object Model (CSSOM)                                      & CSS-OM & 15    & 8,193   & 12.6\%   & 0 \\
      % DeviceOrientation Event Specification                       &         & 2     & 0       & 0.0\%    & 0 \\
      % Directory Upload                                            &         & 1     & 0       & 0.0\%    & 0 \\
      DOM, Level 1 - Specification                                  & DOM1   & 47    & 9,139   & 1.8\%    & 0 \\
      DOM, Level 2 - Core Specification                             & DOM2-C & 31    & 8,951   & 3.0\%    & 0 \\
      DOM, Level 2 - Events Specification                           & DOM2-E & 7     & 9,077   & 2.7\%    & 0 \\
      DOM, Level 2 - HTML Specification                             & DOM2-H & 11    & 9,003   & 4.5\%    & 0 \\
      DOM, Level 2 - Style Specification                            & DOM2-S & 19    & 8,835   & 4.3\%    & 0 \\
      DOM, Level 2 - Traversal and Range Specification              & DOM2-T & 36    & 4,590   & 33.4\%   & 0 \\
      DOM, Level 3 - Core Specification                             & DOM3-C & 10    & 8,495   & 3.9\%    & 0 \\
      DOM, Level 3 - XPath Specification                            & DOM3-X & 9     & 381     & 79.1\%   & 0 \\
      DOM Parsing and Serialization                                 & DOM-PS & 3     & 2,922   & 60.7\%   & 0 \\
      % Encoding                                                    &         & 2     & 1       & 0.0\%    & 0 \\
      % Encrypted Media Extensions                                  &         & 13    & 11      & 11.1\%   & 0 \\
      execCommand                                                   & EC     & 12    & 2,730   & 24.0\%   & 0 \\
      File API                                                      & FA     & 9     & 1,991   & 58.0\%   & 0 \\
      Fullscreen API                                                & FULL   & 9     & 383     & 79.9\%   & 0 \\
      Geolocation API                                               & GEO    & 4     & 174     & 13.1\%   & 0 \\
      % Geometry Interfaces Module, Level 1                         &         & 30    & 0       & 0.0\%    & 0 \\
      % HTML: Broadcasting to other browsing contexts               &         & 2     & 1       & 1.0\%    & 0 \\
      HTML: Channel Messaging                                       & H-CM   & 4     & 5,018   & 77.4\%   & 0 \\
      HTML: Web Storage                                             & H-WS   & 8     & 7,875   & 29.2\%   & 0 \\
      HTML                                                          & HTML   & 195   & 8,980   & 4.3\%    & 0 \\
      HTML: History Interface                                       & H-HI   & 6     & 1,729   & 18.7\%   & 0 \\
      % HTML 5.1                                                    &         & 6     & 3       & 50.0\%   & 0 \\
      % HTML Editing APIs                                           &         & 0     & 0       & 0.0\%    & 0 \\
      % Media Capture from DOM Elements                             &         & 2     & 0       & 0.0\%    & 0 \\
      Media Source Extensions                                       & MSE    & 8     & 1,616   & 37.5\%   & 0 \\
      % MediaStream Recording                                       &         & 10    & 0       & 0.0\%    & 0 \\
      % Navigation Timing                                           &         & 25    & 68      & 29.7\%   & 0 \\
      % Page Visibility (2\textsuperscript{nd} Edition)             &         & 4     & 0       & 0.0\%    & 0 \\
      Performance Timeline                                          & PT     & 2     & 4,690   & 75.8\%   & 0 \\
      Performance Timeline, Level 2                                 & PT2    & 1     & 1,728   & 93.7\%   & 0 \\
      % Pointer Lock                                                &         & 7     & 18      & 100\%    & 0 \\
      % Proximity Events                                            &         & 2     & 18      & 100\%    & 0 \\
      Selection API                                                 & SEL    & 14    & 2,575   & 36.6\%   & 0 \\
      Selectors API, Level 1                                        & SLC    & 6     & 8,674   & 7.7\%    & 0 \\
      % Service Workers                                             &         & 13    & 0       & 0.0\%    & 0 \\
      % Shadow DOM                                                  &         & 1     & 0       & 0.0\%    & 0 \\
      % The Screen Orientation API                                  &         & 9     & 40      & 100\%    & 0 \\
      Timing control for script-based animations                    & TC     & 1     & 3,568   & 76.9\%   & 0 \\
      % Tracking Preference Expression (DNT)                        &         & 1     & 0       & 0.0\%    & 0 \\
      UI Events Specification                                       & UIE    & 8     & 1,137   & 56.8\%   & 0 \\
      % URL                                                         &         & 6     & 5       & 80.0\%   & 0 \\
      User Timing, Level 2                                          & UTL    & 4     & 3,325   & 33.7\%   & 0 \\
      DOM4                                                          & DOM4   & 3     & 5,747   & 37.6\%   & 0 \\
      % WebVTT: The Web Video Text Tracks Format                    &         & 1     & 0       & 0.0\%    & 0 \\
      % Ambient Light Sensor API                                    &         & 1     & 18      & 100\%    & 0 \\
      Non-Standard                                                  & NS     & 65    & 8,669   & 24.5\%   & 0 \\
    \bottomrule
  \end{tabular}
  \caption{Popularity and blockrate for the web standards that are used on at least 1\% of the Alexa 10k
or have at least one associated CVE advisory in the last three years.\\
\textbf{Columns one and two} list the name and abbreviation of the standard.\\
\textbf{Column three} gives the number of features (methods and properties) from that standard that we were able to instrument.\\
\textbf{Column four} includes the number of pages that used at least one feature from the standard, out of the entire Alexa 10k.\\
\textbf{Column five} shows the number of sites on which \textit{no features} in the standard executed in the presence of advertising and tracking blocking extensions (given that the website executed \textit{at least one feature} from the standard in the default case), divided by the number of pages where at least one feature from the standard was executed.  In other words, how often the blocking extensions prevented all features in a standard from executing, given at least one feature would have been used.\\
\textbf{Column six} shows the number of CVEs associated with this standard's implementation
in Firefox within the last three years.
}
  \label{fig:megatable}
\end{table*}

